MirrorMark: Generalizable Mirrored Sampling for Multi-bit LLM Watermarking

As large language models (LLMs) become integral to applications such as question answering and content creation, reliable content attribution has become increasingly important. Watermarking is a promising approach, but most existing methods either provide only binary signals or achieve multi-bit embedding by distorting the generation distribution. We propose MirrorMark, a generalizable mapping-centric approach for multi-bit LLM watermarking. MirrorMark separates the symbol mapping rule from the base watermarking sampler and maps each symbol to a mod-1 mirroring transformation of a detector-reproducible pseudorandom object, such as sampling values or permutation ranks. A binary-tokenizer analysis shows that complementary mappings yield larger matched--mismatched score gaps than independent-key or shift-based mappings. When composed with a distortion-free base sampler, MirrorMark preserves the token probability distribution by design and maintains text quality in practice. To support practical payload embedding, we introduce a Context-Anchored Balanced Scheduler (CABS), which balances token assignments across message positions while localizing edit effects. We further provide theoretical EER analyses for two representative sampler instantiations. Experiments show that MirrorMark achieves strong detectability and bit accuracy while maintaining text quality comparable to non-watermarked generation.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract and introduction state the main contributions, including the mapping-centric view, mod-1 mirroring, CABS, theoretical EER analysis, and empirical evaluation. The claims are supported by the theoretical analysis in Sections~\ref{sec:binary_tokenizer_mapping} and~\ref{sec:theoretical_eer}, and the empirical results in Section~\ref{sec:evaluation}.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper discusses limitations in the robustness evaluation, especially that reliable payload recovery under strong paraphrasing remains open. The paper also notes assumptions in the theoretical EER analysis, including asymptotic approximations and approximate token-level independence, with empirical validation in Appendix~\ref{app:token_independence}.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper provides assumptions, derivations, and proofs for the binary-tokenizer score gaps, mod-1 mirroring motivation, distortion-freeness, and EER analysis in Appendices~\ref{app:binary_mapping_gap},~\ref{motivation_mod1},~\ref{Distortion-freeness}, and~\ref{app:theoretical_eer}. Supporting lemmas are collected in Appendix~\ref{lemmas}.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper specifies the evaluated models, datasets, sampling settings, token lengths, payload sizes, baselines, detection metrics, robustness attacks, and default CABS parameters in Section~\ref{sec:evaluation} and Appendix~\ref{setup}. The algorithms for CABS scheduling, encoding, and decoding are provided in Appendices~\ref{cabs_scheduling_algo}--\ref{cabs_decoder}.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}.
    \item[] Justification: The paper describes the algorithms, datasets, models, and experimental settings needed to reproduce the results. The current submission does not include a public code release, but we plan to release the code upon publication. The experiments use publicly available datasets and models, and the implementation details are described in the appendix.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Appendix~\ref{setup} specifies the datasets, models, sampling settings, CABS parameters, tournament layers, detector training data split, optimizer, learning rate, batch size, and training epochs. The main evaluation settings are summarized in Section~\ref{sec:evaluation}.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper reports 90\% bootstrap confidence intervals for perplexity in the main quality comparison tables. Detection metrics are computed on fixed evaluation sets of 500 paired watermarked and non-watermarked samples using the same protocol for all methods; we report these deterministic aggregate metrics rather than per-run error bars.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Appendix~\ref{setup} reports the main compute resource used in the experiments, including that each Bayesian detector is trained on a single A100 GPU and takes approximately two hours. The remaining experiments mainly consist of text generation, watermark detection, and metric computation using the specified open-weight models and datasets.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work is a watermarking method intended to support provenance detection and responsible use of LLM-generated text. The experiments use public datasets and public or commonly used language models, and the paper does not involve human subjects or private data.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper motivates watermarking as a tool for provenance, accountability, and mitigation of synthetic-content misuse. It also discusses robustness limitations, including degraded payload recovery under paraphrasing, which is important for understanding deployment risks.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not release a new high-risk pretrained model, image generator, or scraped dataset. The work proposes a watermarking method and evaluates it using existing public datasets and models.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper properly cites the existing datasets and models used in the experiments, including C4, ELI5, XL-Sum, LLaMA-2-7B, and Gemma-7B-it. These assets are publicly available, and our use follows their intended research use and terms of access.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not introduce or release a new dataset, pretrained model, or benchmark asset. The main contribution is an algorithmic watermarking method.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing experiments or research with human subjects.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve human subjects, crowdsourcing, or participant studies, so IRB approval is not applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA{}.
    \item[] Justification: LLMs were used only for writing assistance, including grammar, spelling, and wording edits. This usage did not affect the core methodology, scientific rigor, or originality of the research.

\end{enumerate}
